Soft Actor-Critic-based Control Barrier Adaptation for Robust Autonomous Navigation in Unknown Environments

Motion planning failures during autonomous navigation often occur when safety constraints are either too conservative, leading to deadlocks, or too liberal, resulting in collisions. To improve robustness, a robot must dynamically adapt its safety constraints to ensure it reaches its goal while balancing safety and performance measures. To this end, we propose a Soft Actor-Critic (SAC)-based policy for adapting Control Barrier Function (CBF) constraint parameters at runtime, ensuring safe yet non-conservative motion. The proposed approach is designed for a general high-level motion planner, low-level controller, and target system model, and is trained in simulation only. Through extensive simulations and physical experiments, we demonstrate that our framework effectively adapts CBF constraints, enabling the robot to reach its final goal without compromising safety.

==> approach_old.tex <==
\section{Approach}\label{sec:approach}
\textbf{rewrite this with a motivating example}
We propose an SAC-based control barrier adaptation scheme which learns how to adapt the $\alpha$ parameter in \eqref{eq:cbf_const} to improve contour tracking performance in cluttered, unknown environments without the need for any manual tuning of the ZCBF. Data were collected as state transitions $\bm{\zeta}$ into a replay buffer $\mathcal{D}$ during simulated trials. This data were then used to train the SAC model in learning the adaptation function $\hat{f}_\alpha(\bm{s}_k)$ given the current SAC state $\bm{s}_k$. Fig.~\ref{fig:approach_diagram} shows the outline of our approach. The motion planner policy $\Pi$ produces a $C^2$-continuous, time parameterized trajectory $\bm{r}(t) \in \mathbb{R}^2$, which is then sent to a Model Predictive Controller (MPC) incorporating ZCBF constraints as in \eqref{eq:cbf_const} along the predictive horizon $\{\bm{x}_i\}$ to prevent collisions with obstacles. At each control cycle, $\hat{f}(\bm{s}_k)$ is used to adapt the current $\alpha$ value to ensure the vehicle makes progress towards its final goal while also promoting safety. Consider the case shown in Fig.~\ref{fig:planner_demonstration}, where the vehicle is navigating through a cluttered unknown environment. \textbf{add and elaborate on motivating example}. In the following sections, we describe in detail our SAC-based $\alpha$ parameter adaptation framework, starting with a description of the MPC formulation used for this work.
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=.98\textwidth]{main/figs/block_diagram_horiz.png}
    \caption{Block diagram for both the offline training stage and online solver failure prediction and recovery framework.}
    \label{fig:approach_diagram}
\end{figure*}
\begin{figure}[ht!]
    \centering
	\subfigure[]{\includegraphics[width=0.23\textwidth]{main/figs/demonstration_no_cbf.png}\label{fig:no_cbf_2}}
	\subfigure[]{\includegraphics[width=0.23\textwidth]{main/figs/demonstration_const_cbf.png}\label{fig:with_cbf_1}}
    \quad\quad\quad
    \subfigure[]{\includegraphics[width=0.23\textwidth]{main/figs/demonstration_with_sac.png}\label{fig:no_cbf_1}} 
    \subfigure[]{\includegraphics[width=0.23\textwidth]{main/figs/demo_with_sac_graph.png}\label{fig:cbf}} 
    \caption{Put a figure here showing a case where FASTER causes robot to crash into obstacle due to slight intersect with obstacle. Then show how using the CBF would have saved the vehicle from crashing.}
	\label{fig:planner_demonstration}
\end{figure}
% \begin{figure*}[ht!]
%     \centering
%     \subfigure[]{\includegraphics[width=0.233\textwidth]{main/figs/without_cbf_1.png}\label{fig:no_cbf_1}} 
% 	\subfigure[]{\includegraphics[width=0.234\textwidth]{main/figs/without_cbf_2.png}\label{fig:no_cbf_2}}
% 	\subfigure[]{\includegraphics[width=0.24\textwidth]{main/figs/with_cbf_1.png}\label{fig:with_cbf_1}}
% 	\subfigure[]{\includegraphics[width=0.237\textwidth]{main/figs/with_cbf_2.png}\label{fig:with_cbf_2}}
%     \caption{Put a figure here showing a case where FASTER causes robot to crash into obstacle due to slight intersect with obstacle. Then show how using the CBF would have saved the vehicle from crashing.}
% 	\label{fig:planner_demonstration}
% \end{figure*}
% \subsection{Model Predictive Contour Control}
% Model Predictive Contour Control (MPCC) is a type of Optimal Control Problem (OCP) designed to precisely track a predefined, time-parameterized trajectory (or contour) $\bm{r}(t; [t_o,T_r]) = \left[x_r(t) \enspace y_r(t)\right]^T$  \cite{lam2010mpcc}. In this work, the contour is a $C^2$-continuous curve that defines how the vehicle's reference position evolves over time. The cost function for the MPCC is defined as:

% \begin{align}
%     J = & \sum_{k=0}^{N-1} \norm{\bm{x}_k-\bm{x}_r(k\Delta t)}^2_{\bm{Q}} + \sum_{k=0}^{N-2} \norm{\bm{u}_k-\bm{u}_r(k\Delta t)}^2_{\bm{R}} \nonumber \\
%     & + \sum_{k=0}^{N-3} \norm{\bm{u}_{k+1}-\bm{u}_k}^2_{\bm{M}},
% \end{align}

% where $\bm{Q}$, $\bm{R}$, and $\bm{M}$ are cost weighting matrices for state space error, input error, and control regulation respectively, $N$ is the number of steps in the MPC horizon, $\Delta t$ is the MPC time-step, $\bm{x}_k \in \mathcal{X}$ is the robot state for the $k$th prediction step, $\bm{u}_k \in \mathcal{U}$ is the $k$th control input, and $\bm{u}_r$ is the reference trajectory, which is defined as $\bm{u}_r(\cdot)=\left[\norm{\ddot{\bm{r}}(\cdot)} \enspace \omega_r(\cdot) \right]$, where $\omega_r$ is the reference angular velocity, and is defined by:
% \begin{equation}
%     \omega_{r}(t) = \frac{\ddot{\bm{r}}^\perp(t) \cdot \dot{\bm{r}}(t) }{\norm{\dot{\bm{r}}(t)}^2}.
% \end{equation}

% To define the system state $\bm{x}_k$, we consider a modified discrete-time, unicycle model with SE$(2)$ pose $\left[x_k,y_k,\theta_k\right] \in \mathcal{X} \subset \mathbb{R}^2 \times [-\pi, \pi]$, and velocity $v_k \in \mathbb{R}$:
% \begin{equation}\label{eq:unicycle_dynamics}
%     \bm{x}_{k+1} = \begin{bmatrix}
%         x_k \\
%         y_k \\
%         \theta_k \\
%         v_k \\
%         \theta^e_k \\
%         y^e_k
%     \end{bmatrix} +
%     \Delta t\left(\begin{bmatrix}
%         v_k \cos(\theta_k) \\
%         v_k \sin(\theta_k) \\
%         0 \\
%         0 \\
%         -\omega_{r}(k\Delta t) \\
%         v_k \sin(\theta^e_k)
%     \end{bmatrix} + 
%     \begin{bmatrix}
%         0 & 0 \\
%         0 & 0 \\
%         0 & 1 \\
%         1 & 0 \\
%         0 & 1 \\
%         0 & 0 
%     \end{bmatrix}
%     \begin{bmatrix}
%         a_k \\
%         \omega_k
%     \end{bmatrix}\right),
% \end{equation} 
% where $\bm{u}_k = \left[a_k \enspace \omega_k\right]$ is the input vector, wth $a_k, \omega_k \in \mathbb{R}$ representing the linear acceleration and angular velocity respectively. $\left[x_k,y_k,\theta_k\right] \in \mathcal{X} \subset \mathbb{R}^2 \times [-\pi, \pi]$ is the SE$(2)$ pose of the vehicle, $v_k \in \mathbb{R}$ is the velocity, and $\theta^e_k, y^e_k \in \mathbb{R}$ are the heading and cross-track error to the current reference $\bm{r}(k\Delta t)$ respectively. The latter two terms, $\theta^e_k$ and $y^e_k$ (illustrated in Fig.~\ref{fig:state_illustration}) are necessary for the MPC to track $\bm{r}(\cdot)$ accurately, and are defined as:
% % $\bm{u_k}=\left[a_k \enspace \omega_k\right]^T \in \mathbb{R}^2$ is the input with acceleration $a_k$ and angular velocity $\omega_k$. For contour control, we include in the model $\theta^e_k$ and $y^e_k$, which are the heading error and cross-track-error respectively between the vehicle and target trajectory (or contour) $\bm{r}(\cdot)$. Together, $y^e_k$ and $\theta^e_k$ define the contouring error, and can be expressed as:
% \begin{align}
%     y^e_k = & \left(y_k-y_r(k\Delta t)\right)\cos\left(\theta_{r}(k\Delta t)\right) \nonumber \\
%     & - \left(x_k-x_{r}(k\Delta t)\right)\sin\left(\theta_{r}(k\Delta t)\right) \nonumber \\
%     \theta^e_k &= \theta_k - \theta_{r}(k\Delta t) , \enspace \theta_{r} = \atantwo\left(\frac{\dot{y}_{r}(k\Delta t)}{\dot{x}_{r}(k\Delta t)}\right).
% \end{align}
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.98\linewidth]{example-image-c}
%     \caption{Caption}
%     \label{fig:state_illustration}
% \end{figure}
% With the state defined, the OCP is then formulated as:
% % Additionally, $\omega_{r}(t)=\dot{\theta_r}(t)$ is the angular velocity associated with a point along $\bm{r}(t)$:
% % where $\bm{Q}$, $\bm{R}$, and $\bm{M}$ are positive definite weighting matrices, $\bm{x}_r(\cdot)=\left[x_r(\cdot) \enspace y_r(\cdot) \enspace \theta_r(\cdot) \enspace \norm{\dot{\bm{r}}(\cdot)} \enspace 0 \enspace 0\right]$ is the state reference and $\bm{u}_r(\cdot)=\left[\norm{\ddot{\bm{r}}(\cdot)} \enspace \omega_r(\cdot)\right]$ is the input reference. 
% \begin{equation}\label{eq:ocp_no_cbf}
% \begin{aligned}
%     & \underset{\bm{x}, \bm{u}}{\text{argmin}}
%     & & J(\bm{x}, \bm{u}, \bm{r}) \\
%     & \text{subject to}
%     & & \bm{x}_0 = \bm{x}(0) \\
%     & & & \bm{x}_{k+1} = f(\bm{x}_k) + g(\bm{x}_k)\bm{u}_k \\
%     & & & \bm{x}_k \in \mathcal{X}, \enspace \bm{u_k} \in \mathcal{U}
% \end{aligned}
% \end{equation}
% where $\bm{x}(0)$ is the initial state of the vehicle at the start of the control cycle.
\subsection{CBF Formulation}
While the proposed SAC $\alpha$ adaptation scheme is designed to work for any system model where the ZCBF $h(\cdot)$ has relative degree $1$, in this work we focus on a second-order unicycle model. The system state consists of $\text{SE}(2)$ pose $[x,y,\theta] \in \mathcal{X} \subset \mathbb{R}^2 \times [-\pi, \pi]$ and velocity $v \in \mathbb{R}$:
\begin{equation}\label{eq:unicycle_dynamics}
    \dot{\bm{x}} =
    \begin{bmatrix}
        v \cos(\theta) \\
        v \sin(\theta) \\
        0 \\
        0
    \end{bmatrix} + 
    \begin{bmatrix}
        0 & 0 \\
        0 & 0 \\
        0 & 1 \\
        1 & 0
    \end{bmatrix}
    \begin{bmatrix}
        a \\
        \omega
    \end{bmatrix},
\end{equation} 
where $\bm{u} = \left[a \enspace \omega\right]$ is the input vector, with $a, \omega \in \mathbb{R}$ representing the linear acceleration and angular velocity respectively.

\subsection{Augmenting MPCC with CBFs}\label{sec:mpc_cbf_augmentation}
As illustrated in Fig.~\ref{fig:planner_demonstration}, tracking a trajectory with the OCP in \eqref{eq:ocp_no_cbf} lead the vehicle into unsafe states where collisions with obstacles become more likely. To promote safer trajectory tracking, we add a ZCBF constraint following \eqref{eq:cbf_const} at each time-step of the OCP to keep the vehicle from colliding with obstacles, augmenting the OCP formulation in \eqref{eq:ocp_no_cbf} to:
\begin{equation}\label{eq:ocp_with_cbf}
\begin{aligned}
    & \underset{\bm{x}, \bm{u}}{\text{argmin}}
    & & J(\bm{x}, \bm{u}, \bm{r}) \\
    & \text{subject to}
    & & \bm{x}_0 = \bm{x}(0) \\
    & & & \bm{x}_{k+1} = f(\bm{x}_k) + g(\bm{x}_k)\bm{u}_k \\
    & & & L_fh(\bm{x_k}) + L_gh(\bm{x_k})\bm{u_k} + \alpha h(\bm{x_k})\geq 0 \\
    & & & \bm{x}_k \in \mathcal{X}, \enspace \bm{u_k} \in \mathcal{U}
\end{aligned}
\end{equation}

In order to use the ZCBF constraint for obstacle avoidance, the safe set $\mathcal{C}$ and barrier function $h(\bm{x})$ must be set appropriately. For the system in \eqref{eq:unicycle_dynamics}, we define $\mathcal{C}$ as the set of states where the distance $d_o(x,y)$ between the vehicle's center $(x,y)$ and nearest obstacle is larger than the vehicle's minimum circumscribing radius $r_v$:
\begin{equation}
\mathcal{C} = \{\bm{x} \in \mathcal{X} \; | \; d_o(x, y) - r_v > 0\},
\end{equation}
% where $d_o(p_x,p_y)$ is the distance from the robot to the nearest obstacle, and $r_c$ is the minimum circumscribing circle containing the vehicle's footprint. 
With this definition of $\mathcal{C}$, the ZCBF is formulated as proposed in  \cite{ames2017zcbf,li2023cbf}:
\begin{equation}\label{eq:h_func_def}
    h(\bm{x}) = d_o(x,y) \exp{\left\{\nabla d_o(x, y) \cdot \bm{e}_{\theta} - vd_2\right\}}
\end{equation}
where $\nabla d_o(x,y) = [\frac{\partial d_o}{\partial x} \; \frac{\partial d_o}{\partial y}$] is the spatial gradient of $d_o(x,y)$, $\bm{e}_{\theta} = [\cos \theta \; \sin \theta]$ is the unit orientation vector of the vehicle, and $d_2 \in \mathbb{R}^+$ is a user-defined parameter. \textbf{add about signed dist field}

\subsection{Learning CBF Alpha Dynamics}\label{subsec:learning_cbf_sac}
As illustrated in Fig.\textbf{CITE FIG}, using a constant $\alpha$ parameter is insufficient for general navigation tasks because the required level of conservatism varies as the vehicle navigates through a cluttered, unknown environment. When approaching dense obstacle regions, a careful balance between conservatism and aggression is required to negotiate obstacles without collision.

To achieve this dynamic adjustment, the $\alpha$ parameter of the ZCBF constraint in \eqref{eq:cbf_const} can be adapted at runtime, allowing the CBF-MPC to adjust its behavior according to its current state and surroundings. Specifically, a higher $\alpha$ value relaxes the ZCBF constraint, thereby expanding the safe set and enabling more aggressive maneuvers. Conversely, a lower $\alpha$ value contracts the safe set, restricting the vehicle to a more confined safe set. To accomplish this runtime adjustment, we train an offline SAC model $\hat{f}_\alpha$ to learn how to adapt $\alpha$ as the vehicle navigates through its environment. To perform real-time adjustment, we utilize an SAC model, $\hat{f}_\alpha$, which learns to adapt $\alpha$ via the following update equation:
\begin{equation}\label{eq:alpha_update}
    \alpha_{k+1} = \alpha_k + \Delta t * \hat{f}_\alpha (\bm{s}_k).
\end{equation}
In this way we use the SAC model to learn the derivative of $\alpha$ rather than the value of $\alpha_{k+1}$ directly, since empirically this was found to provide smoother $\alpha$ parameter updates, thus leading to smoother resultant motion. 

\subsubsection{SAC Model}
The SAC model is a state-of-the-art, off-policy algorithm that has grown in popularity for real-world robotic reinforcement learning \cite{haarnoja2019sac}. A key feature of SAC is the objective function, which aims to maximize expected return while simultaneously maximizing the entropy of the stochastic policy $\pi_\theta$:
\begin{equation}\label{eq:sac_return}
    J(\pi) = \mathop{\mathbb{E}}_{\tau \sim \pi}\sum_{k=0}^\infty \left[ \gamma^k ( R(\bm{s}_k, a_k, \bm{s}_{k+1}) + \beta H(\pi_\theta(\cdot | \bm{s}_k))\right],
\end{equation}
where $\gamma \in (0, 1]$ is a discount factor on future rewards $R(\cdot)$, $\bm{\tau} = \left(\bm{s}_0, a_0, \bm{s}_1, a_1, \dots \right)$ is a sequence of states $\bm{s}_k$ and actions $a_k$ in the environment, $H(x)=-\log(P(x))$ is the entropy term, and $\beta$ is a fixed trade-off coefficient hand-tuned by the user. However, in this work, we use a variant of SAC which automatically adjusts $\beta$ during training. This dual objective encourages a balance between exploration -- encouraging the vehicle to explore new states -- and exploitation -- maximizing the expected return. By incorporating entropy regularization, SAC prevents $\pi_\theta$ from converging to sub-optimal local minima, while also improving sample efficiency and policy stability.

As the vehicle navigates through its environment, it adds a collection of state transition tuples $\bm{\zeta}_k = (\bm{s}_{k-1}, a_{k-1}, r_{k-1}, \bm{s}_k, d_k)$ to a replay buffer $\mathcal{D}$ of maximum size $N_d$, where $r_{k-1}$ is the transition reward and $d_k$ indicates whether $\bm{s}_k$ is a terminal state (i.e., collision or reach final goal). During training, the SAC model learns three deep neural networks: the (actor) policy $\pi_\theta$ along with two (critic) Q-functions $Q_{\phi_1}$ and $Q_{\phi_2}$, parameterized by $\theta$, $\phi_1$, and $\phi_2$ respectively. To update the networks, SAC uses transitions stored in $\mathcal{D}$ to perform mini-batch stochastic gradient descent, minimizing the following loss functions for $\phi_i$ and $\theta$ respectively:
\begin{equation}\label{eq:sac_loss_functions}
\begin{aligned}
    L(\phi_i, \mathcal{D}) &= \mathop{\mathbb{E}}_{\bm{\zeta}_k \sim D} \left[\left( Q_{\phi_i}(\bm{s}_{k-1},a_k)-y(r_{k-1},\bm{s}_k,d_k) \right)^2 \right] \\
    L(\theta, \mathcal{D}) &= \mathop{\mathbb{E}}_{\substack{\bm{s_k}\sim\mathcal{D} \\ a_k\sim\pi_\theta}} \left[-\beta H\left(\pi_\theta(a_k,\bm{s}_k)\right) -\min_{j=1,2} Q_{\phi_j}(\bm{s}_k,a_k)\right].
\end{aligned}
\end{equation}
Here $y(\cdot)$ is the target for the critic functions and is computed from the received reward and the target value of the next state-action pair, incorporating entropy regularization to encourage exploration. For more details, we refer the reader to \cite{haarnoja2019sac}.

% For training, a navigation stack consisting of the motion planner $\Pi$ and CBF-MPC as defined in \eqref{eq:ocp_with_cbf} were deployed in simulation to populate the replay buffer $\mathcal{D}$ with a collection of state transition tuples $\{\bm{s}_{k-1}, a_k, r_k, \bm{s}_k, d_k\}_{k=1}^|\mathcal{D}|$, where $r$ is the transition reward and $d$ denotes if $\bm{s}_k$ is a terminal state (i.e., collision or reach final goal). To collect the transitions, we use the BARN dataset from \cite{perille2020barn}, which contains $300$ worlds of increasing difficulty, along with the ability to generate new worlds. For this work, we generate $90$ worlds, $40$ for training and $50$ for testing. During data collection, a Clearpath Jackal was deployed to navigate an assigned goal 

% To generate $\mathcal{D}$, we use the BARN dataset from \cite{perille2020barn}, which contains $300$ worlds of increasing difficulty, along with the ability to generate new worlds. For this work, we generate $90$ total new training worlds, $40$ for training and $50$ for testing \textbf{discuss difficulty spread?}. During the data collection stage, a Clearpath Jackal was deployed to navigate an assigned goal position $10m$ in front of the vehicle's initial position. At each control cycle of the ZCBF-MPC, the vehicle recorded the state transition into $\mathcal{D}$. After a terminal state was reached (i.e., collision or reached goal), the SAC model was updated via mini-batch gradient descent using experiences sampled from $\mathcal{D}$.

\subsubsection{SAC For $\alpha$ Adaptation}
To promote feasibility of the ZCBF constraint in \eqref{eq:cbf_const} when using the SAC model for $\alpha$ adaptation, the state representation $\bm{s}_k$ at timestep $k$ for the SAC model includes all relevant system and environment variables necessary for computing $h(\cdot)$ as in \eqref{eq:h_func_def}, along with the value of $h(\cdot)$ itself. Additionally, to encourage the consistent progress towards the final goal and prevent the vehicle from getting stuck in local minima, a progress term $\rho$ is included. 

To define $\rho$, we first determine $t^*$, the time associated with the closest point along the trajectory $\bm{r}(\cdot)$ to the vehicle's current $xy$-position:
\begin{equation}
    t^* = \arg\min_{t\in [0, T_r]} \norm{r(t) - \begin{bmatrix} x \\ y \end{bmatrix} }.
\end{equation}
The progress term $\rho$ is then given by the ratio of $t^*$ to the total trajectory duration $T_r$: 
\begin{equation}
    \rho = \frac{t^*}{T_r}.
\end{equation}
Thus, the full state vector $\bm{s}_k$ is defined as follows:
\begin{equation}
s_k=\left[\theta_k \enspace v_k \enspace a_k \enspace \omega_k \enspace d_o(x_k,y_k) \enspace \gamma_d(x_k,y_k) \enspace \rho_k \enspace \alpha_k \enspace h_k \right]^T, 
\end{equation}
where $\gamma_d(\cdot)$ denotes the heading to the closest obstacle, and is defined as $\gamma_d(x,y)=\atantwo(\frac{\partial d_o}{\partial y}, \frac{\partial d_o}{\partial x})$. Using this definition of the state vector, the SAC model contains knowledge of several salient features, like the relative vehicle position and heading with respect to the closest obstacle in the environment, along with the progress being made along the current trajectory.

With the state defined, the reward function $R(\bm{s}_{k-1}, a_{k-1}, \bm{s}_k)$ is constructed to encourage vehicle safety during navigation to the final goal while also promoting the satisfaction of the ZCBF constraint. The reward is defined by:
\begin{equation}
    R(\bm{s}_{k-1}, a_k, \bm{s}_k) = \mu_d d_o + \mu_\rho \rho - \mu_r \dot{\alpha}^2 - \mu_b b(\alpha) - \mu_h \psi(h),
\end{equation}
where the $\mu_d, \mu_\rho, \mu_r, \mu_b, \mu_h \in \mathbb{R}^+$ are weighting parameters for each component of the reward function. 

The $d_o$ term encourages the vehicle to maintain a safe distance away from obstacles and imposes a large negative reward in the event of a collision. While this term encourages the vehicle to avoid obstacles, relying on it alone can lead to situations where the vehicle receives positive rewards even if it becomes trapped in local minima. To address this issue, the $\rho$ term rewards progress along the current trajectory $\bm{r}(t)$ towards the final goal.

The term $\dot{\alpha}$ functions as a regularization component, penalizing excessive adjustments in the $\alpha$ parameter to promote stability in its control. The function $b(\alpha)$ imposes a penalty if $\alpha \not \in [\alpha^-, \alpha^+]$, where $\alpha^-$ and $\alpha^+$ denote the the predefined minimum and maximum bounds for $\alpha$, respectively.

Finally, $\psi(h)$ penalizes adjustments to $\alpha$ that lead to violations of \eqref{eq:cbf_const}, thus encouraging $h(\cdot)$ to remain non-negative and, as a result keep, the OCP in \eqref{eq:ocp_with_cbf} feasible. This comprehensive reward structure effectively balances the objectives of safe navigation with consistent progression towards the final goal.

% Specifically, in this work the SAC model $\hat{f}_\alpha$ was trained to output the derivative $\dot{\alpha}$ based on current observations $\bm{\xi}_k$, including the current value $\alpha_k$. To this end, the update for $\alpha$ is as follows:
% \begin{equation}
%     \alpha_{k+1} = \alpha_k + \Delta t * \hat{f}_\alpha(\bm{\xi}_k, \alpha_k).
% \end{equation}

% maybe mention something about using the database here instead of openAI gym?
\subsubsection{SAC Training}
For training, a navigation stack consisting of the planning policy $\Pi$ and CBF-MPC as defined in \eqref{eq:ocp_with_cbf} were deployed in a collection of simulation worlds. For this work, we used the BARN dataset \cite{perille2020barn}, which contains $300$ worlds of increasing difficulty, along with the ability to generate new worlds programmatically. For training the model, we generate $40$ new worlds for training, requiring the vehicle to navigate through each $5$ times.

At each control cycle of the CBF-MPC, the vehicle adds a state transition tuple $\bm{\zeta}_k$ to the replay buffer $\mathcal{D}$, which is implemented using an sqlite3 database in this work. Upon reaching a terminal state (i.e., collision or reached goal), the SAC model is updated by sampling mini-batches from the most recent $N_d$ entries in the replay buffer to perform gradient descent on \eqref{eq:sac_loss_functions}. 


\subsection{Motion Planner Integration}
discuss how we integrate the mpc horizon with CBF into the motion planner. Use initial point from MPC horizon to stitch trajectory.

